A Distributed Computing Perspective of Unconditionally Secure Information Transmission in Russian Cards Problems

The problem of $A$ privately transmitting information to $B$ by a public announcement overheard by an eavesdropper $C$ is considered. To do so by a deterministic protocol, their inputs must be correlated. Dependent inputs are represented using a deck of cards. There is a publicly known signature $(a,b,c)$, where $n = a + b + c + r$, and $A$ gets $a$ cards, $B$ gets $b$ cards, and $C$ gets $c$ cards, out of the deck of $n$ cards. Using a deterministic protocol, $A$ decides its announcement based on her hand. Using techniques from coding theory, Johnson graphs, and additive number theory, a novel perspective inspired by distributed computing theory is provided, to analyze the amount of information that $A$ needs to send, while preventing $C$ from learning a single card of her hand. In one extreme, the generalized Russian cards problem, $B$ wants to learn all of $A$'s cards, and in the other, $B$ wishes to learn something about $A$'s hand.

==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}


\subsection{Topological models for epistemic logic}
\label{sec:prelim:epistemic-logic} % sec:prelim:epistemic-logic
We recap here the new kind of model for epistemic logic based on 
chromatic simplicial complexes, introduced in~\cite{gandalf2018}. 
%\comment{% not room for in conference version to repeat this:
%We will show that these simplicial models are very closely 
%related to the usual Kripke models which are widely used to study the semantics 
%of epistemic logic formulas: there is an equivalence of categories between the
%two structures.
The geometric nature of simplicial complexes allows us to consider higher-dimensional topological
properties of our models, and investigate their meaning in terms of knowledge.
The idea of using simplicial complexes comes from distributed computability~\cite{HerlihyKR:2013,kozlov:2007}.
After describing simplicial models, we explain how to use them in DEL.%ynamic Epistemic Logic. 
%}
%The link with DEL and distributed computing will be developed in the next sections.


\paragraph{Syntax}
Let $\Atom$ be a countable set of atomic propositions and $\Agents$ a finite set of agents.
The language $\mathcal{L}_K$ is generated by the following BNF
grammar:
\[
\varphi ::= p \mid \neg\varphi \mid (\varphi \land \varphi) \mid
K_a\varphi \qquad p \in \Atom,\ a \in \Agents
\]
In the following, we work with $n+1$ agents, and write $\Agents = \{ a_0, \ldots, a_n \}$.

\paragraph{Semantics}
The usual semantics for multi-agent epistemic logic is based on Kripke frames.
The notion of model that we use here, which is based on simplicial complexes,
is merely a reformulation of the usual Kripke models using a different formalism.
The benefits of this reformulation is that it makes
explicit the topological information of Kripke frames. The precise relationship
between the usual Kripke models and our simplicial models is studied thoroughly in~\cite{gandalf2018}.

\begin{definition} [Simplicial complex \cite{kozlov:2007}]
A \emph{simplicial complex} $\langle V, M \rangle$ is given by a set $V$ of \emph{vertices} and a family $M$ of non-empty finite subsets of $V$ called \emph{simplices}, such that
for all $X \in M$, $Y \subseteq X$ implies $Y \in M$. We say that~$Y$ is a \emph{face} of $X$.
\end{definition}

Usually, the set of vertices is implicit and we simply refer to a simplicial complex as $M$. We write $\vertices{M}$ for the set of vertices of $M$. 
%Elements of $\vertices{M}$ (identified with singletons) are called \emph{vertices}.
A vertex $v \in \vertices{M}$ is identified with the singleton $\{v\} \in M$. 
Elements of $M$ are called \emph{simplices}, and those which are maximal w.r.t.\ inclusion are \emph{facets} (or \emph{worlds}),  the set of which  is denoted by $\facets{M}$. 
 The \emph{dimension} of a simplex $X \in M$ is  $|X|-1$. 
 A simplicial complex $M$ is \emph{pure} if all its facets are of the same dimension $n$. In this case,
 we say $M$ is of dimension $n$.
Given a finite set $\Agents$ of agents (that we will represent as colors), a \emph{chromatic simplicial complex} $\la M, \chi \ra$ consists of a simplicial complex $M$ and a coloring map $\chi : \vertices{M} \to \Agents$, such that for all $X \in M$, all the vertices of $X$ have distinct colors.

\begin{definition}[Simplicial map]
\label{def:morphism_of_complexes}
%\begin{definition} [Simplicial maps \cite{kozlov:2007}] 
Let $C$ and $D$ be two simplicial complexes. A \emph{simplicial map} 
$f: C \rightarrow D$ 
maps the vertices of $C$ to vertices of $D$, such that if~$X$ is a simplex of~$C$, $f(X)$ %(the image set
%on the subset of vertices $X$) 
is a simplex of $D$.
A \emph{chromatic simplicial map} between two chromatic simplicial complexes is a simplicial map that preserves colors.
\end{definition}

%
%Let ${\cal S}_A$ be the category of pure chromatic simplicial complexes on $A$, 
%with chromatic simplicial maps for morphisms. 

For technical reasons, we restrict to models where all the atomic propositions
are saying something about some local value held by one particular agent. All the examples 
that we are interested in will fit in that framework. Let $\Values$ be some 
countable set of values, and $\Atom = \{ p_{a,x} \mid a \in \Agents, x \in \Values \}$ 
be the set of \emph{atomic propositions}. Intuitively, $p_{a,x}$ is true if agent 
$a$ holds the value $x$.
%In all our examples, an agent will hold exactly one value, but we do not enforce that.
We write $\Atom_a$ for the atomic propositions concerning agent $a$, that is, 
 $\Atom_a = \{p_{a,x} \mid x\in \Values \}$.

\begin{definition}[Simplicial model]
A \emph{simplicial model} $\cM = \la C, \chi, \ell \ra$ consists of a pure chromatic simplicial 
complex $\la C, \chi \ra$ of dimension $n$, and a labeling $\ell : \vertices{C} \to \mathscr{P}(\Atom)$
that associates with each vertex $v \in \vertices{C}$ a set of atomic propositions concerning agent~$\chi(v)$, i.e., such that $\ell(v) \subseteq \Atom_{\chi(v)}$.
\end{definition}

Given a facet $X = \{v_0, \ldots, v_n\} \in C$, we write $\ell(X) = \bigcup_{i=0}^n \ell(v_i)$.
A \emph{morphism} of simplicial models $f : \cM \to \cM'$ is a chromatic simplicial map that preserves the labeling: $\ell'(f(v)) = \ell(v)$ (and $\chi$).
We denote by ${\cal SM}_{\Agents,\Atom}$ the category of simplicial models over the set of 
agents $\Agents$ and atomic propositions $\Atom$.

\begin{definition}\label{semantFormulas}
We define the truth of a formula $\varphi$ in some epistemic state $(\cM,X)$ with $\cM=\la C, \chi, \ell \ra$ a simplicial model, $X \in \facets{C}$ a facet of $C$ and
$\varphi \in \Lcal_K(\Agents,\Atom)$.
The satisfaction relation, determining when a formula is true in an
epistemic state, is defined as:

\begin{tabular}{lcl}
$\cM,X \models p$ & \quad if \quad & $p \in \ell(X)$\\
$\cM,X \models \neg \varphi$ & \quad if \quad & $\cM,X \not\models \varphi$\\
$\cM,X \models \varphi \wedge \psi$ & \quad if \quad & $\cM,X \models \varphi
\mbox{ and } \cM,X \models \psi$\\
$\cM,X \models K_a \varphi$ & \quad if \quad & $\mbox{for all } Y \in \cF(C), a \in \chi(X \cap Y) \mbox{ implies } \cM,Y \models \varphi$\\
\end{tabular}
\end{definition}

\subsection{Equivalence with Kripke models}

Simplicial models can be seen as a different formalism to talk about Kripke models.
Indeed, as explained in~\cite{gandalf2018}, every simplicial model can be associated with an equivalent Kripke model. Conversely, every Kripke model which is \emph{proper} and \emph{local} can be associated with an equivalent simplicial model.
We recall these facts in Theorem~\ref{thm:equiv-model} below, which is proved in~\cite{gandalf2018}.

A \emph{Kripke frame} $M=\la S, \sim \ra$ over a set $\Agents$ of agents consists of  a set
of states $S$ and a family of equivalence relations on $S$, written $\sim_a$ for every $a \in \Agents$.
Two states $u, v \in S$ such that $u \sim_a v$ are said to be \emph{indistinguishable} by $a$.
A Kripke frame is \emph{proper} if any two states can be distinguished by at least one agent.
%Notice that being proper means that the intersection
%of all equivalence relations~$\sim_a$ is the identity; this may reveal
%interesting parallels with distributed knowledge (a formula that is true
%in all states in the intersection relation), see e.g. \cite{FHMVbook}.
%
Let $M=\la S, \sim \ra$ and $N=\la T,\sim' \ra$ be two Kripke frames over the same set of agents $\Agents$.
A \emph{morphism} from  $M$ to $N$ is a function~$f$ from $S$ to $T$ such that for all $u, v \in S$, for all $a \in \Agents$, 
$u \sim_a v$ implies $f(u) \sim'_a f(v)$. 

\begin{definition}[Kripke model]
A \emph{Kripke model}  $M = {\la S,\sim,L\ra}$ consists of a Kripke frame
$\la S, \sim \ra$  and a function $L : S \to \mathscr{P}(\Atom)$. %\I{AP}
Intuitively, $L(s)$ is the set of atomic propositions that are true in the state $s$.
\end{definition}

A Kripke model is \emph{proper} if the underlying Kripke frame is proper.
A Kripke model is \emph{local} if for every agent $a \in \Agents$, $s \sim_a s'$ implies
$L(s) \cap \Atom_a = L(s') \cap \Atom_a$, i.e., an agent always 
knows its own values.
%
Let $M=\la S, \sim,L \ra$ and $M'=\la S',\sim',L' \ra$ be two Kripke
models over the same set $\Atom$. A \emph{morphism of Kripke models} $f : M \to M'$
is a morphism of the underlying Kripke frames such that 
$L'(f(s)) =  L(s)$ for every state $s$ in~$S$. 
We write ${\cal KM}_{\Agents, \Atom}$ for the category of local proper Kripke models. 

%\medskip
%We can now extend the two maps $F$ and $G$ of Theorem~\ref{thm:equiv} to an equivalence between simplicial models and Kripke models.

\begin{theorem}[\cite{gandalf2018}]
\label{thm:equiv-model}
${\cal SM}_{\Agents,\Atom}$ and ${\cal KM}_{\Agents,\Atom}$ are equivalent categories.
\end{theorem}

A direct corollary of Theorem \ref{thm:equiv-model} is that Definition~\ref{semantFormulas} agrees with the usual definition of truth on Kripke models (see~\cite{gandalf2018}). 

%Gain  of knowlege
% HOP

\subsection{Topological semantics for Dynamic Epistemic Logic}
\label{sec:prelim_del}
The simplicial models described in Section~\ref{sec:prelim:epistemic-logic}
%\ref{sec:prelim:epistemic-logic} 
can also be used to model Dynamic Epistemic Logic (DEL). DEL is the study of various epistemic logics extended with model-changing operators~\cite{sep-dynamic-epistemic,DEL:2007}.
One such logic is the one based on \emph{action models}~\cite{baltagMS:98}, which are relational structures that can be used to describe a variety of communication actions.

\paragraph{Syntax}
We extend the syntax of epistemic logic with one more construction:
\[
\varphi ::= p \mid \neg\varphi \mid (\varphi \land \varphi) \mid
K_a\varphi \mid [\alpha]\varphi \qquad p \in \Atom,\ a \in \Agents
\]
Intuitively, the formula $[\alpha]\varphi$ means that $\varphi$ is true after some 
\emph{action} $\alpha$ has occurred.
An action can be thought of as an 
announcement made by the environment,
which is not necessarily public, in the sense that
not all  agents receive these announcements.
The semantics of this new operator should be understood as follows (under assumption that~$\alpha$ can be executed in the world $X$):
 \[ \cM,X \models [\alpha] \varphi \quad \text{if} \quad \cM[\alpha],X[\alpha] \models \varphi\]
i.e., the formula $[\alpha] \varphi$ is true in some world $X$ of $\cM$ whenever, on condition that the action $\alpha$ can be executed in world $X$, $\phi$ is true in world $X[\alpha]$ of some new model $\cM[\alpha]$, where the knowledge of each agent has been modified according to the action $\alpha$.


\paragraph{A simplicial complex version of DEL}
To define formally what an action is, we first need to introduce the notion of \emph{action model}.
An action model describes all the possible actions that might happen, as well
as how they affect the different agents.

\begin{definition}
\label{def:actionmodels}
An \emph{action model} is a structure $\cA = \la T,\sim,\pre\ra$,
where~$T$ is a domain of \emph{actions}, such that for
each $a \in \Agents$, $\sim_a$ is an equivalence relation on $T$, and
$\pre : T \to \Lcal_\cK$ is a  function that assigns a
\emph{precondition} formula $\pre(t)$ to each $t \in T$
\end{definition}
 An \emph{action} $\alpha$ is defined as a pair  $(\cA,t)$ where $t \in T$.
 Additionally, in order to keep the action language defined above well-defined, action models must have a \emph{finite} domain $T$.
%
An action model is \emph{proper} if for any two different actions $t, t' \in T$, there is an agent $a \in \Agents$ who can distinguish between them, i.e., $t \not \sim_a t'$.

\begin{definition}[Product update model]
\label{def:produpdate}
Given a simplicial model $\cM = \langle C, \chi, \ell \rangle$ and an action model $\cA = \la T, \sim, \pre \ra$, we define the \emph{product update simplicial model} $\cM[\cA] = \la C[\cA], \chi[\cA], \ell[\cA]  \ra$ as follows. 
Intuitively, the facets of $C[\cA]$ should correspond to pairs $(X,t)$ where $X \in C$ is a world of $\cM$ and $t \in T$ is an action of $\cA$, such that $\cM,X \models \pre(t)$.
Moreover, two such facets $(X,t)$ and $(Y,t')$ should be glued along their $a$-colored vertex whenever $a \in \chi(X \cap Y)$ and $t \sim_a t'$.
Formally, the vertices of $C[\cA]$ are pairs $(v,E)$ where $v \in \cV(C)$ is a vertex of $C$; $E$ is an equivalence class of  $\sim_{\chi(v)}$; and $v$ belongs to some facet $X \in C$ such that there exists $t \in E$ such that $\cM,X \models \pre(t)$.
Such a vertex keeps the color and labeling of its first component: $\chi[\cA](v,E) = \chi(v)$ and $\ell[\cA](v,E) = \ell(v)$.
\end{definition}
%
We can finally state the formal semantics of the formula $[\alpha]\varphi$:
 \[ \cM,X \models [\cA, t] \varphi \qquad \text{if} \qquad \cM,X \models \pre(t) \implies \cM[\cA],(X,t) \models \varphi\]
